Particle propagation in non-trivial backgrounds: a quantum field theory approach

The basic aim of the thesis is the study of the propagation of particles and quasiparticles in non-trivial backgrounds from the quantum field theory point of view. By "non-trivial background" we mean either a non-vacuum state in Minkowski spacetime or an arbitrary state in a curved spacetime. Starting with the case of a flat spacetime, the basic properties of the particle and quasiparticle propagation are analyzed using two different methods other than the conventional mean-field-based techniques: on the one hand, the quantum state corresponding to the quasiparticle excitation is explicitly constructed; on the other hand, the spectral representation of the two-point propagators is analyzed. Both methods lead to the same results: the energy and decay rate of the quasiparticles are determined by the real and imaginary parts of the retarded self-energy respectively. These general results are applied to two particular quantum systems: first, a scalar particle immersed in a thermal graviton bath; second, a simplified atomic model, seizing the opportunity to connect with other statistical and first-quantized approaches. In the second part of the thesis the results are extended to curved spacetime. Working with a quasilocal quasiparticle concept the flat-spacetime results are recovered. In cosmology, within the adiabatic approximation, it is possible to go beyond the flat spacetime results and find additional effects due to the universe expansion. The cosmologically-induced effects are analyzed, obtaining that there might be an additional contribution to the particle decay due to the universe expansion. In the de Sitter case, this additional contribution coincides with the decay rate in a thermal bath in a flat spacetime at the corresponding de Sitter temperature.

==> thermal.tex <==
\chapter{Real-time thermal field theory}\label{app:TFT}

\index{Thermal field theory}


For the benefit of those readers who might be unfamiliar with the
subject we give in this appendix a brief account of those aspects
of real-time thermal field theory which are needed in the paper.
For a complete introduction to the thermal field theory we address
the reader to Refs.~\cite{LandsmanWeert87,DasThermal,LeBellac};
see also Ref.~\cite{CamposHu98} for an approach similar
o ours.

\section{Correlation functions}

In thermal field theory the initial state for the fields is
assumed to be a thermal state at temperature $T=1/\beta$, which is
characterized by a density matrix
\begin{equation}
     \hat\rho = \frac{\expp{- \beta\hat
    H}}{\Tr(\expp{- \beta\hat {H}})},
\end{equation}
where $ \hat{H}$ is the Hamiltonian operator of the system (for
the purposes of this appendix we shall consider a scalar field
$\phi$). The generating functional $Z_{\mathcal C}[j]$ is defined
as
\begin{equation}
    Z_{\mathcal C}[j] = \Tr \left(\hat \rho T_{\mathcal C} \expp{i \int_{\mathcal C} \vd t \int
    \ud[3]{\vect
    x} \hat \phi(x) j(x)}  \right),
\end{equation}
where $\hat \phi(x)$ is the field operator in the Heisenberg
picture, ${\mathcal C}$ is a certain path in the complex $t$
plane, $T_{\mathcal C}$ means ordering along this path and $j(x)$
is a classical external source. By functional differentiation of
the generating functional with respect to $\phi$, path-ordered
correlation functions can be obtained. The generating functional
may be computed in a path-integral representation as
\begin{equation}
    Z_{\mathcal C}[j] = \int \uD \phi \expp{ i  \int_{\mathcal C} \vd t \int
    \ud[3]{\vect x} \left\{ {\mathcal L}[\phi(x)] + j(x) \phi(x)\right\} },
\end{equation}
where ${\mathcal L}$ is the Lagrangian density and the contour
${\mathcal C}$ is now restricted to begin at some initial real
time $t_\mathrm i$ and to end at $t_\mathrm i - i\beta$. The
boundary conditions for the path integral are $\phi(t_\mathrm
i,\vect x) = \phi(t_\mathrm i-i\beta,\vect x)$. Different
elections for ${\mathcal C}$ lead to different approaches to
thermal field theory: a straight line from $t_\mathrm i$ to
$t_\mathrm i - i\beta$ leads to the imaginary-time formalism, and
the contour shown in Fig.~\ref{fig:Path} leads to the real-time
formalism. By choosing $\sigma= 0^+$ our formalism will coincide
with the closed time path (CTP) approach to non equilibrium field
theory \cite{Schwinger61,Keldysh65,ChouEtAl85}. In fact many of
the properties listed below are not limited to the thermal case
but are valid in a more general non equilibrium situation. We
shall try to specify in each case which properties are general and
which ones are particular to the thermal case.

\begin{figure}
    \centering
    \includegraphics{path}
    \caption{Integration contour in the complex-time plane used in the
    real-time approach to thermal field theory. The choice
    $\sigma=0^+$ makes the formalism analogous to the CTP approach to
    field theory.}
    \label{fig:Path}
\end{figure}


If we are interested in real-time correlation functions, the path
along ${\mathcal C}_3$ and ${\mathcal C}_4$ can be usually
neglected once we properly take into account the boundary
conditions of the path integral. If we define $\phi_{1,2}(t,\vect
x)=\phi(t,\vect x)$ and $j_{1,2}(t,\vect x)=j(t,\vect x)$ for $t
\in {\mathcal C}_{1,2}$, and take $t_\mathrm i \to -\infty$ and
$t_\mathrm f\to \infty$ the generating functional can be
reexpressed as $Z_{\mathcal C}[j] = Z_{34} Z[j_1,j_2]$, where
$Z_{34}$ represents the constant contribution from the segments
${\mathcal C}_3$ and ${\mathcal C}_4$ and $Z[j_1,j_2]$ is
\begin{equation}
\begin{split}
    Z[j_1,j_2]= \int \uD \phi_1 \uD \phi_2 & \expp{i\int \ud[4]x
    \left\{ {\mathcal L}[\phi_1(x)] + j_1(x) \phi_1(x)\right\}}
    \\ \times & \expp{ -i\int \ud[4]x \left\{
      {\mathcal L}[\phi_2(x)] + j_2(x)
    \phi_2(x) \right\}}.
\end{split}
\end{equation}
Correlation functions are defined by second functional
differentiation with respect to the external source $j(x)$:
\begin{equation}
    G_{ab}(x,x') =
    \left.\frac{1}{Z[0,0]}\derff{Z[j_1,j_2]}{j^a(x)}{j^b(x)}\right|_{j_1=j_2=0},
\end{equation}
where $a,b = 1,2$. In operator language correlation functions can
be written as
\begin{subequations} \label{CorrFunct}
\begin{align}
    G_{11}(x,x') &= \av{ T \hat\phi(x) \hat\phi(x') }, \\
    G_{12}(x,x') &= \av{ \hat\phi(x) \hat\phi(x') }, \\
    G_{21}(x,x') &= \av{ \hat\phi(x') \hat\phi(x) }, \\
    G_{22}(x,x') &= \av{ \widetilde T \hat\phi(x) \hat\phi(x') },
\end{align}
\end{subequations}
where $(\widetilde T)$ $T$ is the (anti-) time-ordering operator,
and where the average means $\av{\cdots}= \Tr{(\hat\rho \cdots)}$.
Lowercase roman indices are raised and lowered with the ``metric''
$c_{ab}=\mathrm{diag}(1,-1)$. From the above expressions it can be
readily seen that not all correlation functions are independent.
The following relations in Fourier space are a consequence of
Eqs.~\eqref{CorrFunct}:
\begin{subequations} \label{RelG}
\begin{gather}
    G_{11}(p) = G_{22}^*(p), \qquad G_{12}(p)=G_{21}(-p),\\
    G_{11}(p) + G_{22}(p) = G_{12}(p) + G_{21}(p),
\end{gather}
\end{subequations}
where correlation functions in Fourier space are
\begin{equation*}
    G_{ab}(p) = \int \ud[4]{x} \expp{-i p \cdot \Delta}
    G_{ab}(X+\Delta/2,X-\Delta/2),
\end{equation*}
where we have introduced the new variables $\Delta=x-x'$ and
$X=(x+x')/2$ \footnote{In order to avoid cumbersome notation the
same symbol is used for correlators in configuration space and in
Fourier space. Notice that Fourier-transformed propagators depend
on $X$ if the initial state is non homogeneous. Since our primary
concern here is thermal states, which are homogeneous, we do not
indicate explicitly this $X$ dependence.}. Additionally, in the
case of an initial thermal state the following relation, a
consequence of the Kubo-Martin-Schwinger (KMS) formula (equivalent
to the fluctuation-dissipation theorem, in another context), is
also verified:
\begin{equation}
    G_{11}(p) + G_{22}(p) = \expp{-\beta p^0} G_{12}(p) + \expp{\beta p^0}
    G_{21}(p).
\end{equation}
Thus, in thermal field theory the knowledge of just one
correlation function determines all of them.

\index{Propagator!retarded}
\index{Propagator!advanced}

An important correlation function is the retarded propagator,
which is defined as
\begin{equation}
    G_\mathrm R(x,x') = \theta(x^0-x'^0) \av{[\hat
    \phi(x),\hat\phi(x')]},
\end{equation}
and is related to the other correlation functions through
\begin{equation}
    G_\mathrm R(p) = G_{11}(p) - G_{12}(p).
\end{equation}
The retarded propagator has the remarkable property that has well
defined analyticity properties at finite temperature, as opposite
to most other propagators: it is analytic in the upper half of the
complex $p^0$ plane. Furthermore, the retarded propagator is the
one that one naturally obtains from an analytic continuation of
the Euclidian propagator in the imaginary-time formalism
\cite{FetterWalecka}.

\section{Perturbation theory}

Perturbation theory can be organized in a similar way as in the
zero-temperature case, but taking into account that at finite
temperature there are two kind of vertices ($1$ and $2$) and four
kind of propagators ($11$, $12$, $21$ and $22$) which link the two
vertices. Vertices type 2 carry an additional minus sign with
respect to vertices type 1. When computing Feynman diagrams one
has to sum over all possible internal vertices. For a real scalar
field of mass $m$, free propagators are given by
\begin{equation} \label{FreeGT}
\begin{split}
         G_{ab}^{(0)}(p)  &=
        \begin{pmatrix}
            \dfrac{-i}{p^2 + m^2 - i \epsilon} & {2\pi \delta(p^2+m^2) \theta(-p^0)}\\
            { 2\pi \delta(p^2+m^2) \theta(p^0)}
             & \dfrac{i}{p^2 + m^2 + i \epsilon}
        \end{pmatrix} \\ &\quad + 2\pi \delta(p^2+m^2) {n(|p^0|)}
        \begin{pmatrix}
            1 & 1 \\
            1 & 1
        \end{pmatrix},
\end{split}
\end{equation}
where $n(E)$ is the Bose-Einstein distribution function:
\begin{equation}
    n(E) = \frac{1}{1-\expp{\beta E}}.
\end{equation}
Thermal contributions to Feynman diagrams are always finite in the
ultraviolet regime because the Bose-Einstein function acts as a
soft cutoff for momenta larger than the temperature $T$. The
counterterms which renormalize the theory at zero temperature also
renormalize the theory at finite temperature. Note also that the
thermal part of the propagator, which breaks the Lorentz symmetry
through an explicit dependence on $p^0$, is always on shell.

Instead of working with the four propagators $G_{ab}(p)$ in the
thermal case one can reorganize perturbation theory in a way such
that just retarded and advanced propagators are involved
\cite{EijckKobesWeert94}. In this case one has to consider how
Feynman rules are transformed when working with the
retarded/advanced basis.


\section{Self-energy}

In a thermal or, more generally, in a non equilibrium situation,
the self-energy has a matricial structure and is implicitly
defined through the equation
\begin{equation} \label{SDM}
    G_{ab}(p) = G_{ab}^{(0)}(p)+
    G_{ac}^{(0)}(p) [-i\Sigma^{cd}(p)]  G_{db}(p),
\end{equation}
where $G^{(0)}_{ab}(p)$ are the free propagators of the theory.
The $ab$ component of the self-energy can be computed, similarly
to the vacuum case, as the sum of all one-particle irreducible
diagrams with  amputated external legs that begin and end with
type $a$ and type $b$ vertices, respectively.

In general the self-energy components verify the non-perturbative
relations
\begin{subequations} \label{RelSigma}
\begin{gather}
    \Sigma^{11}(p) =- (\Sigma^{22})^*(p), \qquad \Sigma^{12}(p)=\Sigma^{21}(-p)\\
    \Sigma^{11}(p) + \Sigma^{22}(p) =-  \Sigma^{12}(p) -
    \Sigma^{21}(p),
\end{gather}
\end{subequations}
which can be obtained from Eqs.~\eqref{RelG} and \eqref{SDM}. The
following equation is just verified if the initial state is
thermal:
\begin{equation}
    \Sigma^{11}(p) + \Sigma^{22}(p) = -\expp{-\beta p^0} \Sigma^{12}(p) - \expp{\beta p^0}
    \Sigma^{21}(p).
\end{equation}
Thus, all the components of the self-energy can be determined from
knowledge of just one of them. Combining relations
\eqref{RelSigma} we obtain
\begin{equation} \label{cut}
    \Im \Sigma^{11}(p) = \frac{i}{2} [ \Sigma^{12}(p) +
    \Sigma^{21}(p)
    ].
\end{equation}
This last equation can be directly obtained from the cutting rules
at finite temperature.

\index{Self-energy!retarded}
\index{Self-energy!advanced}

A particularly useful combination is the  retarded self-energy,
defined as $\Sigma_\mathrm R(p) = \Sigma^{11}(p) +
\Sigma^{12}(p)$. It  is related to the retarded propagator through
\begin{equation}\label{SigmaAR}
    {G}_\mathrm{R}(p) = \frac{-i}{p^2 + m^2+
    \Sigma_\mathrm{R}(p)}.
\end{equation}
The above relation, which justifies the name of retarded
self-energy for $\Sigma_\mathrm{R}(p)$, can be demonstrated by
expanding the matrix equation \eqref{SDM} and using the relations
\eqref{RelG} and \eqref{RelSigma}. Similar relations hold for thels
advanced propagator $G_\mathrm A(p) = G^*_\mathrm R(p)$ and the
advanced self-energy $\Sigma_\mathrm A(p) = -\Sigma^*_\mathrm
R(p)$. Notice that a diagonal relation such as Eq.~\eqref{SigmaAR}
can be found only for the retarded (or advanced) propagator.


According to \Eqref{cut}, the imaginary part of the retarded
self-energy can be also expressed as
\begin{equation} \label{cutR}
    \Im \Sigma_\mathrm R(p) = \frac{i}{2} [ \Sigma^{21}(p) -
    \Sigma^{12}(p)
    ].
\end{equation}
For a thermal state $\Sigma_\mathrm R(p)$ is related to
$\Sigma^{11}(p)$ through:
\begin{equation}
    \Sigma^\mathrm R(p)  = \Re \Sigma^{11}(p) + \tanh
    \left( \frac{p^0}{2T} \right) \Im \Sigma^{11}(p). \label{SigmaR11}
\end{equation}

